Discontinuity Induced Hopf and Neimark-Sacker Bifurcations in a Memristive Murali-Lakshmanan-Chua Circuit

We report using Clarke's concept of generalised differential and a modification of Floquet theory to non-smooth oscillations, the occurrence of discontinuity induced Hopf bifurcations and Neimark-Sacker bifurcations leading to quasiperiodic attractors in a memristive Murali-Lakshmanan-Chua (memristive MLC) circuit. The above bifurcations arise because of the fact that a memristive MLC circuit is basically a nonsmooth system by virtue of having a memristive element as its nonlinearity. The switching and modulating properties of the memristor which we have considered endow the circuit with two discontinuity boundaries and multiple equilibrium points as well. As the Jacobian matrices about these equilibrium points are non-invertible, they are non-hyperbolic, some of these admit local bifurcations as well. Consequently when these equilibrium points are perturbed, they lose their stability giving rise to quasiperiodic orbits. The numerical simulations carried out by incorporating proper discontinuity mappings (DMs), such as the Poincar\'{e} discontinuity map (PDM) and zero time discontinuity map (ZDM), are found to agree well with experimental observations.

==> epsfsafe.tex <==
%   EPSF.TEX macro file (modified for EPSF images with TIFF preview)
%
%   Written by Tomas Rokicki of Radical Eye Software, 29 Mar 1989.
%   Revised by Don Knuth, 3 Jan 1990.
%   Revised by Tomas Rokicki to accept bounding boxes with no
%	space after the colon, 18 Jul 1990.
%-%   Modified to deal with %%BoundingBox: (at end) as well as TIFF
%-%	preview in EPSF format files, 1993 Jan 23 (see %-% comments).
%
%   TeX macros to include an Encapsulated PostScript graphic.
%   Works by finding the bounding box comment,
%   calculating the correct scale values, and inserting a vbox
%   of the appropriate size at the current position in the TeX document.
%
%   To use with the center environment of LaTeX, preface the \epsffile
%   call with a \leavevmode.  (LaTeX should probably supply this itself
%   for the center environment.)
%
%   To use, simply say
%   \input epsfsafe	  % somewhere early on in your TeX file
%   \epsfbox{filename.ps} % where you want to insert a vbox for a figure
%
%   Alternatively, you can type
%
%   \epsfbox[0 0 30 50]{filename.ps} % to supply your own BB
%
%   which will not read in the file, and will instead use the bounding
%   box you specify.
%
%   The effect will be to typeset the figure as a TeX box, at the
%   point of your \epsfbox command. By default, the graphic will have its
%   `natural' width (namely the width of its bounding box, as described
%   in filename.ps). The TeX box will have depth zero.
%
%   You can enlarge or reduce the figure by saying
%     \epsfxsize=<dimen> \epsfbox{filename.ps}
%   (or
%     \epsfysize=<dimen> \epsfbox{filename.ps})
%   instead. Then the width of the TeX box will be \epsfxsize and its
%   height will be scaled proportionately (or the height will be
%   \epsfysize and its width will be scaled proportiontally).  The
%   width (and height) is restored to zero after each use.
%
%   A more general facility for sizing is available by defining the
%   \epsfsize macro.  Normally you can redefine this macro
%   to do almost anything.  The first parameter is the natural x size of
%   the PostScript graphic, the second parameter is the natural y size
%   of the PostScript graphic.  It must return the xsize to use, or 0 if
%   natural scaling is to be used.  Common uses include:
%
%      \epsfxsize  % just leave the old value alone
%      0pt	   % use the natural sizes
%      #1	   % use the natural sizes
%      \hsize	   % scale to full width
%      0.5#1	   % scale to 50% of natural size
%      \ifnum#1>\hsize\hsize\else#1\fi	% smaller of natural, hsize
%
%   If you want TeX to report the size of the figure (as a message
%   on your terminal when it processes each figure), say `\epsfverbosetrue'.
%
\chardef\quoteleftcode=\catcode96	% remember catcode of `
\catcode96=12				% make sure ` is "ordinary"

\newread\epsffilein    % file to \read
\newif\ifepsffileok    % continue looking for the bounding box?
\newif\ifepsfbbfound   % success?
\newif\ifepsfverbose   % report what you're making?
\newdimen\epsfxsize    % horizontal size after scaling
\newdimen\epsfysize    % vertical size after scaling
\newdimen\epsftsize    % horizontal size before scaling
\newdimen\epsfrsize    % vertical size before scaling
\newdimen\epsftmp      % register for arithmetic manipulation
\newdimen\pspoints     % conversion factor
%
\pspoints=1bp	       % Adobe points are `big'
\epsfxsize=0pt	       % Default value, means `use natural size'
\epsfysize=0pt	       % ditto
%
\def\epsfbox#1{\global\def\epsfllx{72}\global\def\epsflly{72}%
   \global\def\epsfurx{540}\global\def\epsfury{720}%
   \def\lbracket{[}\def\testit{#1}\ifx\testit\lbracket
   \let\next=\epsfgetlitbb\else\let\next=\epsfnormal\fi\next{#1}}%
%
\def\epsfgetlitbb#1#2 #3 #4 #5]#6{\epsfgrab #2 #3 #4 #5 .\\%
   \epsfsetgraph{#6}}%
%
\def\epsfnormal#1{\epsfgetbb{#1}\epsfsetgraph{#1}}%
%
\def\epsfgetbb#1{%
%
%   The first thing we need to do is to open the
%   PostScript file, if possible.
%
\openin\epsffilein=#1
\ifeof\epsffilein\errmessage{I couldn't open #1, will ignore it}\else
%
%   Okay, we got it. Now we'll scan lines until we find one that doesn't
%   start with %. We're looking for the bounding box comment.
%
   {\epsffileoktrue \chardef\other=12
    \def\do##1{\catcode`##1=\other}\dospecials \catcode`\ =10
%-% Neuter some more nasty characters
    \catcode`\^^L=9 \catcode`\^^?=9
    \loop
       \read\epsffilein to \epsffileline
       \ifeof\epsffilein\epsffileokfalse\else
%
%   We check to see if the first character is a % sign;
%   if not, we stop reading (unless the line was entirely blank);
%   if so, we look further and stop only if the line begins with
%   `%%BoundingBox:'.
%
	  \expandafter\epsfaux\epsffileline:. \\%
       \fi
   \ifepsffileok\repeat
   \ifepsfbbfound\else
    \ifepsfverbose\message{No bounding box comment in #1; using defaults}\fi\fi
   }\closein\epsffilein\fi}%
%
%   Now we have to calculate the scale and offset values to use.
%   First we compute the natural sizes.
%
\def\epsfclipstring{}% do we clip or not?  If so,
\def\epsfclipon{\def\epsfclipstring{ clip}}%
\def\epsfclipoff{\def\epsfclipstring{}}%
%
\def\epsfsetgraph#1{%
   \epsfrsize=\epsfury\pspoints
   \advance\epsfrsize by-\epsflly\pspoints
   \epsftsize=\epsfurx\pspoints
   \advance\epsftsize by-\epsfllx\pspoints
%
%   If `epsfxsize' is 0, we default to the natural size of the picture.
%   Otherwise we scale the graph to be \epsfxsize wide.
%
   \epsfxsize\epsfsize\epsftsize\epsfrsize
   \ifnum\epsfxsize=0 \ifnum\epsfysize=0
      \epsfxsize=\epsftsize \epsfysize=\epsfrsize
      \epsfrsize=0pt
%
%   We have a sticky problem here:  TeX doesn't do floating point arithmetic!
%   Our goal is to compute y = rx/t. The following loop does this reasonably
%   fast, with an error of at most about 16 sp (about 1/4000 pt).
%
     \else\epsftmp=\epsftsize \divide\epsftmp\epsfrsize
       \epsfxsize=\epsfysize \multiply\epsfxsize\epsftmp
       \multiply\epsftmp\epsfrsize \advance\epsftsize-\epsftmp
       \epsftmp=\epsfysize
       \loop \advance\epsftsize\epsftsize \divide\epsftmp 2
       \ifnum\epsftmp>0
          \ifnum\epsftsize<\epsfrsize\else
	     \advance\epsftsize-\epsfrsize \advance\epsfxsize\epsftmp \fi
       \repeat
       \epsfrsize=0pt
     \fi
   \else \ifnum\epsfysize=0
     \epsftmp=\epsfrsize \divide\epsftmp\epsftsize
     \epsfysize=\epsfxsize \multiply\epsfysize\epsftmp
     \multiply\epsftmp\epsftsize \advance\epsfrsize-\epsftmp
     \epsftmp=\epsfxsize
     \loop \advance\epsfrsize\epsfrsize \divide\epsftmp 2
     \ifnum\epsftmp>0
	\ifnum\epsfrsize<\epsftsize\else
	   \advance\epsfrsize-\epsftsize \advance\epsfysize\epsftmp \fi
     \repeat
     \epsfrsize=0pt
    \else
     \epsfrsize=\epsfysize
    \fi
   \fi
%
%  Finally, we make the vbox and stick in a \special that dvips can parse.
%
   \ifepsfverbose\message{#1: width=\the\epsfxsize, height=\the\epsfysize}\fi
   \epsftmp=10\epsfxsize \divide\epsftmp\pspoints
   \vbox to\epsfysize{\vfil\hbox to\epsfxsize{%
      \ifnum\epsfrsize=0\relax
        \special{PSfile=#1 llx=\epsfllx\space lly=\epsflly\space
            urx=\epsfurx\space ury=\epsfury\space rwi=\number\epsftmp
            \epsfclipstring}%
      \else
        \epsfrsize=10\epsfysize \divide\epsfrsize\pspoints
        \special{PSfile=#1 llx=\epsfllx\space lly=\epsflly\space
            urx=\epsfurx\space ury=\epsfury\space rwi=\number\epsftmp\space
            rhi=\number\epsfrsize \epsfclipstring}%
      \fi
      \hfil}}%
\global\epsfxsize=0pt\global\epsfysize=0pt}%
%
%   We still need to define the tricky \epsfaux macro. This requires
%   a couple of magic constants for comparison purposes.
%
{\catcode`\%=12 \global\let\epsfpercent=%\global\def\epsfbblit{%BoundingBox}}%
%
%   So we're ready to check for `%BoundingBox:' and to grab the
%   values if they are found.
%
\long\def\epsfaux#1#2:#3\\{\ifx#1\epsfpercent
   \def\testit{#2}\ifx\testit\epsfbblit
      \epsfgrab #3 . . . \\%
      \epsffileokfalse
      \global\epsfbbfoundtrue
%-% Don't stop if line does not start with %.  May be (at end) or binary stuff
%  \fi\else\ifx#1\par\else\epsffileokfalse\fi\fi}%
   \fi\else\ifx#1\par\else\fi\fi}%
%
%   Here we grab the values and stuff them in the appropriate definitions.
%
\def\epsfempty{}%
\def\epsfgrab #1 #2 #3 #4 #5\\{%
\global\def\epsfllx{#1}\ifx\epsfllx\epsfempty
      \epsfgrab #2 #3 #4 #5 .\\\else
   \global\def\epsflly{#2}%
   \global\def\epsfurx{#3}\global\def\epsfury{#4}\fi}%
%
%   We default the epsfsize macro.
%
\def\epsfsize#1#2{\epsfxsize}
%
%   Finally, another definition for compatibility with older macros.
%
\let\epsffile=\epsfbox

\catcode`\`=\quoteleftcode		% restore previous catcode

==> epstopdf/README <==
$Id: README 32701 2014-01-17 18:09:54Z karl $
This file is public domain.  (Originally written by Karl Berry, 2009.)

This is the README for the epstopdf script distribution.

Primary distribution point: http://mirror.ctan.org/support/epstopdf/
  (list of mirrors at: http://ctan.org/mirrors)

Home page: http://tug.org/epstopdf/

Run epstopdf --help for the usual list of options, examples, etc.

Mailing list for bugs and discussion: http://lists.tug.org/tex-k
When reporting bugs, please include an input file and command line
options, so the problem can be reproduced.

-------------------------------------------------------------------------
The test-binary and test-bin2 files were supplied by Akira Kakuto and
Reinhard Kotucha.  They contain binary data.  They are public domain.

The test-binhdr* files were supplied by Martin von Gagern, constructed
as follows.  They contain binary junk before the EPS starts.  We also
use these to test different line endings.  These files are public domain.

{ echo -e '%Some\000binary\001comment'; dot -Tps <<< 'digraph{a->b}'; }
  > test-binhdr-lf.eps
tr $'\n' $'\r' <test-binhdr-lf.eps >test-binhdr-cr.ps
unix2dos <test-binhdr-lf.eps >test-binhdr-cr.ps


==> epstopdf/epstopdf.1 <==
.TH EPSTOPDF 1 "28 May 2016"
.\" $Id: epstopdf.1 41288 2016-05-29 16:50:38Z karl $
.SH NAME
epstopdf, repstopdf \- convert an EPS file to PDF
.SH SYNOPSIS
\fBepstopdf\fP [\fIoptions\fP] [\fIepsfile\fP]
.SH DESCRIPTION
By default, \fBepstopdf\fP converts the input PostScript file to PDF,
using Ghostscript.
.PP
\fBEpstopdf\fP transforms the Encapsulated PostScript file \fIepsfile\fP
(or standard input) so that it is guaranteed to start at the 0,0
coordinate, and it sets a page size exactly corresponding to the
BoundingBox.  Thus, the result needs no cropping, and the PDF MediaBox
is correct.  
.PP
PJL commands at the start of a file are removed.  DOS EPS binary files
(TN 5002) are supported.
.PP
If the bounding box in the input is incorrect, of course there will
be resulting problems.
.SH OPTIONS
Options may start with either "\fB-\fP" or "\fB--\fP", and may be
unambiguously abbreviated.  It is best to use the full option name in
scripts to avoid possible collisions with new options in the future.
.PP
General script options:
.IP "\fB--help\fP
display help message and exit
.IP "\fB--version\fP
display version information and exit
.IP "\fB--outfile\fP=\fIfile\fP"
write result to \fIfile\fP.  If this option is not given, and
\fB--nogs\fP or \fB--filter\fP is specified, write to standard output;
otherwise, the default is to construct the output file name by replacing
any extension in the input file with `.pdf'.
.IP "\fB--\fP[\fBno\fP]\fBdebug\fP"
write debugging info (default: false).
.IP "\fB--\fP[\fBno\fP]\fBexact\fP"
scan ExactBoundingBox (default: false).
.IP "\fB--\fP[\fBno\fP]\fBfilter\fP"
read standard input and (unless \fB--outfile\fP is given) write standard
output (default: false).
.IP "\fB--\fP[\fBno\fP]\fBgs\fP"
run Ghostscript (default: true).  With \fB--nogs\fP, output (to standard
output by default) the PostScript that would normally be converted; that
is, the input PostScript as modified by \fBepstopdf\fP.
.IP "\fB--\fP[\fBno\fP]\fBhires\fP"
scan HiresBoundingBox (default: false).
.IP "\fB--restricted\fP=\fIval\fP"
turn on restricted mode (default: [true for repstopdf, else false]);
this forbids the use of \fB--gscmd\fP and other options and imposes
restrictions on the input and output file names according to the values
of openin_any and openout_any (see the Web2c manual, http://tug.org/web2c).
.PP
Options for Ghostscript (more info below):
.IP "\fB--gscmd\fP=\fIval\fP"
pipe output to \fIval\fP (default: [\fBgswin32c\fP on Windows, else \fBgs\fP])
.IP "\fB--gsopt\fP=\fIval\fP"
include \fIval\fP as one argument in the gs command (can be repeated).
.IP "\fB--gsopts\fP=\fIval\fP"
split \fIval\fP at whitespace and include each resulting word as an
argument in the gs command (can be repeated).
.IP "\fB--autorotate\fP=\fIval\fP"
set AutoRotatePages (default: None); recognized \fIval\fP choices:
None, All, PageByPage.  For EPS files, PageByPage is equivalent to All.
.IP "\fB--\fP[\fBno\fP]\fBcompress\fP"
use compression in the output (default: true); if turned off, passes
.IR -dUseFlateCompression=false .
.IP "\fB--device\fP=\fIdev\fP"
use -sDEVICE=\fIdev\fP (default: pdfwrite); not allowed in restricted mode.
.IP "\fB--\fP[\fBno\fP]\fBembed\fP"
embed fonts (default: true); passes
.I -dMaxSubsetPct=100 -dSubsetFonts=true -dEmbedAllFonts=true.
.IP "\fB--\fP[\fBno\fP]\fBgray\fP"
grayscale output (default: false); passes
.I -sColorConversionStrategy=Gray -dProcessColorModel=/DeviceGray.
.IP "\fB--pdfsettings\fP=\fIval\fP"
use -dPDFSETTINGS=/\fIval\fP (default is `prepress' if \fB--embed\fP,
else empty); recognized \fIval\fP choices: screen, ebook, printer,
prepress, default.
.IP "\fB--\fP[\fBno\fP]\fBquiet\fP"
use -q, a.k.a. -dQUIET (default: false).
.IP "\fB--res\fP=\fIdpi, dpi\fPx\fIdpi\fP"
set image resolution (default: [use gs default]); ignored if
\fB--debug\fP is set.
.IP "\fB--\fP[\fBno\fP]\fBsafer\fP"
use -d(NO)QUIET (default: true).
.PP
In addition to the specific options above, additional options to be used
with gs can be specified with either or both of the two cumulative
options \fB--gsopts\fP and \fB--gsopt.\fP
.PP
\fB--gsopts\fP takes a single string of options, which is split at
whitespace, each resulting word then added to the gs command line
individually.
.PP
\fB--gsopt\fP adds its argument as a single option to the gs command
line.  It can be used multiple times to specify options separately,
and is necessary if an option or its value contains whitespace.
.PP
In restricted mode, options are limited to those with names and values
known to be safe.  Some options taking booleans, integers or fixed
names are allowed, those taking general strings are not.

.SH EXAMPLES
These examples all equivalently convert `test.eps' to `test.pdf':
.nf
epstopdf test.eps
cat test.eps | epstopdf --filter >test.pdf
cat test.eps | epstopdf -f -o=test.pdf
.fi
.PP
Example for using HiResBoundingBox instead of BoundingBox:
.nf
epstopdf --hires test.eps
.fi
.PP
Example for \fBepstopdf\fP's attempt at correcting PostScript:
.nf
$program --nogs test.ps >testcorr.ps
.fi
.PP
In all cases, you can add \fB--debug\fP (\fB-d\fP) to see more about
what \fBepstopdf\fP is doing.
.SH BUGS
The case of "%%BoundingBox: (atend)" when input is not seekable (e.g.,
from a pipe) is not supported.
.PP
Report bugs in the program or this man page to tex-k@tug.org.  When
reporting bugs, please include an input file and the command line
options specified, so the problem can be reproduced.
.SH SEE ALSO
\fBgs\fP(1),
\fBpdfcrop\fP(1).
.PP
The epstopdf LaTeX package, part of the oberdiek bundle, which automates
running this script on the fly under TeX: http://ctan.org/pkg/epstopdf-pkg.
.SH AUTHOR
Originally written by Sebastian Rahtz, for Elsevier Science, with
subsequent contributions from Thomas Esser, Gerben Wierda, Heiko
Oberdiek, and many others.  Currently maintained by Karl Berry.
.PP
Man page originally written by Jim Van Zandt.
.PP
epstopdf home page: http://tug.org/epstopdf.
.PP
You may freely use, modify and/or distribute this file.

